On the Robustness of Fairness Practices: A Causal Framework for Systematic Evaluation

Machine learning (ML) algorithms are increasingly deployed to make critical decisions in socioeconomic applications such as finance, criminal justice, and autonomous driving. However, due to their data-driven and pattern-seeking nature, ML algorithms may develop decision logic that disproportionately distributes opportunities, benefits, resources, or information among different population groups, potentially harming marginalized communities. In response to such fairness concerns, the software engineering and ML communities have made significant efforts to establish the best practices for creating fair ML software. These include fairness interventions for training ML models, such as including sensitive features, selecting non-sensitive attributes, and applying bias mitigators. But how reliably can software professionals tasked with developing data-driven systems depend on these recommendations? And how well do these practices generalize in the presence of faulty labels, missing data, or distribution shifts? These questions form the core theme of this paper.

==> Sections/Algorithm1.tex <==
\begin{algorithm}[!bht]
\scriptsize
\DontPrintSemicolon
    \KwIn{Dataset $\mathcal{A}$, ML algorithm $\mathcal{M}$, Default HP $h\textsubscript{0}$, 
    Non-sensitive attributes $\mathcal{NP}$, Sensitive attributes $\mathcal{P}$, type of analysis $\tau$,
    Feature selection method $f\_s$, the step size $stp\_size$, HP constraints $\mathcal{S}$, Max. HP search $N$,
    and Timeout $\mathcal{T}$.
    }
    $\mathcal{G}$, $edges\_list$ $\gets$ \texttt{CausalDiscovery}($\mathcal{A}$) \Comment{Causal Discovery} \\
    $\mathcal{W^G}$ $\gets$ \texttt{Stan}($\mathcal{G}$, $edges\_list$) \Comment{Causal Inference} \\
    $\mathcal{A\textsubscript{0}}$ $\gets$ \texttt{Generate}($\mathcal{G}$, $\mathcal{W^G}$)\\
    $EOD\textsubscript{0}$, $Acc\textsubscript{0}$ $\gets$ \texttt{Train}($\mathcal{M}$, $h\textsubscript{0}$, $\mathcal{A\textsubscript{0}}, \mathcal{P}$)\\
    % $EOD_{max}$ $\gets$  $EOD\textsubscript{0}$\\

    $Found$, $t$, $t_0$ $i$, $\mathcal{G}_0$, $\mathcal{W^G_\textsubscript{0}}$ $\gets$ \texttt{False}, 0, 0, \texttt{time}(), $\mathcal{G}$, $\mathcal{W^G}$
    
    \While{$t \leq \mathcal{T}$}{
        $\mathcal{G\textsubscript{1}}$,  $\mathcal{W^G_\textsubscript{1}}$ $\gets$ \texttt{perturb}($\mathcal{G\textsubscript{0}}$, $\mathcal{W^G_\textsubscript{0}}$, $\mathcal{G}$, $\mathcal{W^G}$, $stp\_size$ )\\
        $\mathcal{A\textsubscript{1}}$ $\gets$ \texttt{Generate}($\mathcal{G\textsubscript{$1$}}$,  $\mathcal{W^G_\textsubscript{1}}$ )\\
        \If{$\tau$ == Drop\_Analysis}{
            $\mathcal{A\textsubscript{dropped}}$  $\gets$  \texttt{Drop}($\mathcal{A\textsubscript{1}}$, $\mathcal{P}$) \\
            $EOD_1$, $Acc\textsubscript{1}$ $\gets$ \texttt{Train}($\mathcal{M}$, $h_0$, $\mathcal{A\textsubscript{dropped}}$, $\mathcal{P}$)\\
            \If{$EOD_0$ > $EOD_1$}{
                 $\mathcal{G\textsubscript{$\mathcal{P}$}}$ $\gets$ $\mathcal{G\textsubscript{1}}$

                $Found$ $\gets$ \texttt{True}
            }
        }
        \If{$\tau$ == featureSelection\_Analysis}{
            // {\color{black}f\_s: \texttt{Random}, \texttt{Kbest}, \texttt{Fpr}, or \texttt{Percentile}}
                        
            $\mathcal{A\textsubscript{1}}$  $\gets$  \texttt{f\_s}($\mathcal{A\textsubscript{1}}$, $\mathcal{NP}$) \\

            $EOD_{1}$, $Acc_{1}$ $\gets$ \texttt{Train}($\mathcal{M}$, $h_0$,   $\mathcal{A\textsubscript{1}}$, $\mathcal{P}$)\\
            
            \If{$EOD_0$ > $EOD_1$}{
                 $\mathcal{G\textsubscript{$\mathcal{NP}$}}$ $\gets$ $\mathcal{G\textsubscript{1}}$

                $Found$ $\gets$ \texttt{True}
            }
        }   
        \If{$\tau$ == $\mathcal{HP}$\_Analysis}{
            
            \If{i == 0}{    
                \texttt{$HP_0$}, $EOD_0$  $\gets$ \texttt{HP\_Search}($\mathcal{M}$, $\mathcal{A\textsubscript{0}}$, $\mathcal{S}$, $h_0$, $N$)
                                
                $HP\_Imp_0$ $\gets$  \texttt{SHAP}$((HP_0, EOD_0))$          
            }
            
            \For{$h \in HP_0$}{
                $EOD\textsubscript{1}$, $Acc_{1}$ $\gets$ \texttt{Train}($\mathcal{M}$, $h$,  $\mathcal{A\textsubscript{1}}$, $\mathcal{P}$)\\
                $HP_1$.\texttt{add}($h$)
            }
           $HP\_Imp_1$ $\gets$ \texttt{SHAP}$((HP_1, EOD_1))$
           
           $distance$ $\gets$ \texttt{Distance}($HP\_Imp_0$,  $HP\_Imp_1$)
           
           \If{$distance$ > 2}{
                $\mathcal{G\textsubscript{$\mathcal{HP}$}}$ $\gets$  $\mathcal{G\textsubscript{$1$}}$

                $Found$ $\gets$ \texttt{True}
            }  
        }
        \If{{\it Found}}{
            Break
        }
        \If{\texttt{Interesting($\mathcal{G\textsubscript{1}}$,$\mathcal{G\textsubscript{0}}$)}}{
            $\mathcal{G\textsubscript{0}}$, $\mathcal{W^G_\textsubscript{0}}$ $\gets$ $\mathcal{G\textsubscript{1}}$, $\mathcal{W^G_\textsubscript{1}}$
        }
        $t$, $i$ $\gets$ \texttt{time}() - $t_0$, $i + 1$

    }
    return  $\mathcal{G_\textsubscript{0}}$, $\mathcal{G\textsubscript{$\mathcal{P}$}}$,  $\mathcal{G\textsubscript{$\mathcal{NP}$}}$, $\mathcal{A\textsubscript{1}}$,  $\mathcal{G\textsubscript{$\mathcal{HP}$}}$, $HP_1$
   
\caption{Causal Search}
\label{alg:algorithm1}
\end{algorithm}

==> Sections/Table_RQ1_validation.tex <==

\setlength{\tabcolsep}{15pt} % Default value: 6pt
\begin{table}[t!]
    \centering
    \caption{Comparing data generation techniques.
      Legend:
      \textbf{Algorithm}: Generating method,
      \textbf{FID}: Fréchet inception distance,
      \textbf{KL-D}: Kullback–Leibler divergence,
      \textbf{LG-D}: logistic regression detection,
      \textbf{Acc}: accuracy difference,
      \textbf{F1} : Downstream F1 loss.     
    }
    \label{tab:RQ0}
    \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{|l|c|c|c|c|c|} 
      \hline
          
    & &\multicolumn{3}{c|}{\textbf{Similarity}} & \textbf{ML Perf} \\ \cline{3-6} 
     \textbf{Dataset} & \textbf{Algorithm} & FID & KL-D & LG-D   & F1 loss \\
    \hline
    \multirow{3}{*}{Adult}&GES&.02 & \textbf{.93}&.74  & .03 \\
    &SIMY&\textbf{.01} & \textbf{.93}&\textbf{.78}  & \textbf{.01} \\
    &RND&.11 & .19&.01 & .25 \\
    \hline
    \multirow{3}{*}{Compas}&PC&\textbf{.08} & .97&.61  & \textbf{.0}\\
    &GES&\textbf{.08} & \textbf{.98}&\textbf{.63 } & \textbf{.0} \\
    &RND&.30 & .76&.02 & .51 \\
    \hline
    \multirow{3}{*}{Bank}&GES&\textbf{.02} & \textbf{.88}&\textbf{.73}  & \textbf{.0} \\
    &RND&.20 & .12&.01  & .26 \\
    \hline
    \multirow{3}{*}{Law School}&GES&\textbf{.09 }& \textbf{.93}&\textbf{.54 } & .16 \\
    &SIMY&.13 & .77&.35  & \textbf{.09} \\
    &RND&.13 & .31&.15  & .39 \\
     \hline
    \multirow{3}{*}{Students}&PC&\textbf{.09 }& \textbf{.93}&\textbf{.54 } & .16 \\
    &SIMY&.13 & .77&.35  & \textbf{.09} \\
    &RND&.13 & .31&.15  & .39 \\
    \hline
     \multirow{3}{*}{Heart}&GES&\textbf{.09} & .90&\textbf{.22 } & .18 \\
    &RND&.10 & .87&.02  & .76 \\
    \hline    
    \end{tabular}
}
\end{table}


==> Sections/Table_RQ2_OOD.tex <==

% {\footnotesize
\begin{table*}[!t]
\caption{Impacts of Sensitive \& Non-Sensitive Feature Selection on Fairness under Distribution Shifts.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multirow{2}{*}{\textbf{Model}}&\multirow{2}{2.5em}{\textbf{Dataset}}  &\multicolumn{4}{| c |}{\hfil\textsc{SelectKBest~\cite{KBest}}} & \multicolumn{4}{| c |}{\hfil\textsc{SelectFpr~\cite{SelectFpr}}}  &\multicolumn{4}{| c |} {\hfil\textsc{SelectPercentile~\cite{SelectPercentile}}} & \multicolumn{4}{| c |}{\hfil\textsc{DropSensParam}} \\\cline{ 3-18}
&&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff} &\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}    \\
\hline

\multirow{6}{*}{LR}&\multirow{2}{*}{Adult}& \multirow{2}{*}{1} & \textbf{0.06} & 0.0 & 0.0 & \multirow{2}{*}{0} & 0.02 & 0.0 & 0.0 & \multirow{2}{*}{1} & \textbf{0.4} & -0.06 & -0.11 & \multirow{2}{*}{4} & \textbf{0.24} & -0.24 & -0.02\\
&&  & -0.27 & -0.02 & -0.03 &   & -0.01 & -0.0 & 0.0 &  & -0.33 & -0.13 & -0.08 &  & -0.26 & -0.02 & -0.02 \\\cline{2-18}


&\multirow{2}{*}{Compas} & \multirow{2}{*}{3} & \textbf{0.08} & -0.0 & -0.0 &  \multirow{2}{*}{0} & \textbf{0.08} & -0.0 & -0.0 & \multirow{2}{*}{2} & \textbf{0.06} & -0.02 & -0.01 & \multirow{2}{*}{3} & \textbf{0.09} & 0.05 & 0.0\\
&&  & -0.01 & -0.0 & 0.0 &   & -0.01 & -0.0 & 0.0 &  & -0.04 & -0.02 & -0.0 &  & -0.02 & 0.0 & 0.0 \\\cline{2-18}


&\multirow{2}{*}{Bank}& \multirow{2}{*}{1} & \textbf{0.04} & -0.04 & -0.04 &  \multirow{2}{*}{0} & 0.01 & 0.0 & 0.0 & \multirow{2}{*}{1} & \textbf{0.41} & -0.01 & -0.0 & \multirow{2}{*}{1} & \textbf{0.12} & 0.12 & -0.12\\
&&  & -0.12 & -0.02 & -0.07 &   & -0.01 & 0.0 & 0.0 &  & -0.28 & -0.08 & -0.37 &  & -0.06 & -0.01 & -0.02 \\\cline{2-18}


&\multirow{2}{*}{Law School}&  \multirow{2}{*}{2} & 0.04 & -0.01 & 0.0 &  \multirow{2}{*}{0} & 0.0 & 0.0 & 0.0 & \multirow{2}{*}{2} & 0.02 & -0.0 & 0.0 & \multirow{2}{*}{2} & 0.03 & 0.01 & 0.0\\
&&  & 0.01 & -0.0 & 0.0 &   & -0.0 & 0.0 & 0.0 &  & -0.02 & -0.01 & -0.01 &  & 0.01 & 0.0 & 0.0 \\\cline{2-18}


&\multirow{2}{*}{Student}&  \multirow{2}{*}{0} & 0.01 & -0.0 & 0.0 &  \multirow{2}{*}{0} & 0.01 & -0.0 & 0.0 & \multirow{2}{*}{8} & 0.01 & -0.01 & -0.0 & \multirow{2}{*}{8} & 0.01 & 0.0 & 0.0\\
&&  & -0.01 & -0.01 & -0.0 &   & -0.01 & -0.01 & -0.0 &  & -0.01 & -0.02 & -0.01 &  & -0.01 & -0.0 & 0.0 \\\cline{2-18}


&\multirow{2}{*}{Heart}&  \multirow{2}{*}{0} & \textbf{0.16} & -0.0 & 0.0 &  \multirow{2}{*}{0} & \textbf{0.12} & 0.0 & 0.0 & \multirow{2}{*}{0} & \textbf{0.26} & -0.07 & -0.06 & \multirow{2}{*}{1} & \textbf{0.16} & -0.15 & 0.02\\
&&  & -0.06 & -0.05 & -0.04 &   & -0.01 & -0.03 & -0.06 &  & 0.01 & -0.1 & -0.08 &  & -0.02 & 0.0 & 0.0 \\
\hline

\multirow{6}{*}{DT}&\multirow{2}{*}{Adult}& \multirow{2}{*}{1} & 0.0 & 0.0 & 0.0  & \multirow{2}{*}{3} & 0.0 & 0.0 & 0.0  & \multirow{2}{*}{2} &  \textbf{0.23} & -0.31 & -0.48  & \multirow{2}{*}{0} &0.0 & 0.0 & 0.0 \\
&&  & -0.04 & -0.07 & -0.08 & & 0.0 & 0.0 & 0.0 & & -0.52 & -0.36 & -0.36 & & 0.0 & 0.0 & 0.0
  \\\cline{2-18}



&\multirow{2}{*}{Compas}& \multirow{2}{*}{2} & \textbf{0.03} & -0.04 & 0.01 & \multirow{2}{*}{0} &\textbf{0.03} & -0.04 & 0.01  & \multirow{2}{*}{0} &  \textbf{0.01} & -0.07 & 0.0 & \multirow{2}{*}{0} & \textbf{0.07} & -0.01 & 0.0 \\
&&  &  -0.06 & -0.03 & 0.02 & & -0.05 & -0.04 & 0.01 & & -0.08 & -0.06 & 0.01 & & -0.01 & -0.01 & 0.01 \\\cline{2-18}



&\multirow{2}{*}{Bank}& \multirow{2}{*}{1} &   \textbf{0.04} & -0.11 & -0.06  & \multirow{2}{*}{4} & 0.02 & -0.08 & -0.04 & \multirow{2}{*}{3} & \textbf{0.34} & -0.12 & -0.06 & \multirow{2}{*}{3} &0.02 & -0.01 & -0.01 \\
&&  & -0.03 & -0.07 & -0.04 & & -0.01 & -0.0 & -0.0 & & -0.09 & -0.29 & -0.6 & & -0.03 & -0.01 & -0.01 \\\cline{2-18}



&\multirow{2}{*}{Law School}& \multirow{2}{*}{6} & 0.0 & 0.0 & 0.0 & \multirow{2}{*}{2} & 0.0 & 0.0 & 0.0  & \multirow{2}{*}{1} &  0.03 & -0.17 & -0.09 & \multirow{2}{*}{0} & 0.0 & 0.0 & 0.0 \\
&&  & 0.0 & 0.0 & 0.0 & & 0.0 & 0.0 & 0.0 & & -0.03 & -0.2 & -0.13 & & 0.0 & 0.0 & 0.0  \\\cline{2-18}


&\multirow{2}{*}{Student}& \multirow{2}{*}{1} &  0.0 & 0.0 & 0.0  & \multirow{2}{*}{1} & 0.0 & -0.03 & -0.02 & \multirow{2}{*}{} & 0.01 & -0.1 & -0.06  & \multirow{2}{*}{1} & 0.0 & 0.0 & 0.0 \\
&&  &  -0.0 & 0.0 & 0.0 & & -0.0 & -0.03 & -0.02 & & -0.01 & -0.09 & -0.06 & & 0.0 & 0.0 & 0.0  \\\cline{2-18}



&\multirow{2}{*}{Heart}& \multirow{2}{*}{0} &  0.02 & -0.05 & -0.04  & \multirow{2}{*}{0} & 0.01 & -0.03 & -0.03  & \multirow{2}{*}{1} &  \textbf{0.11} & -0.24 & -0.24  & \multirow{2}{*}{2} & 0.0 & 0.0 & 0.0 \\
&&  &  -0.01 & -0.03 & -0.05 & & -0.0 & -0.0 & -0.0 & & -0.16 & -0.32 & -0.23 & & -0.0 & 0.0 & 0.0  \\\cline{2-18}

\hline
\multirow{6}{*}{SVM}&\multirow{2}{*}{Adult}& \multirow{2}{*}{6} &  \textbf{0.14} & -0.02 & -0.02  & \multirow{2}{*}{1} & \textbf{0.03} & -0.0 & -0.03  & \multirow{2}{*}{2} &  \textbf{0.48} & -0.02 & -0.14  & \multirow{2}{*}{2} & \textbf{0.41} & 0.0 & -0.03 \\
&&  & -0.19 & -0.02 & -0.05 & & -0.06 & -0.0 & -0.0 & & -0.24 & -0.06 & -0.02 & & -0.2 & -0.01 & -0.02  \\\cline{2-18}


&\multirow{2}{*}{Compas}& \multirow{2}{*}{4} & 0.02 & -0.0 & 0.0 & \multirow{2}{*}{2} &0.02 & -0.0 & 0.0  & \multirow{2}{*}{3} &  -0.01 & -0.02 & -0.0  & \multirow{2}{*}{4} & 0.02 & 0.0 & 0.0\\
&&& -0.02 & -0.0 & 0.0 & & -0.02 & -0.0 & 0.0 & & -0.05 & -0.02 & -0.0 & & -0.01 & 0.0 & 0.0  \\\cline{2-18}

&\multirow{2}{*}{Bank}& \multirow{2}{*}{3} & \textbf{0.04} & -0.02 & -0.02 & \multirow{2}{*}{3} & \textbf{0.04} & -0.03 & -0.02  & \multirow{2}{*}{3} &  \textbf{0.08} & -0.01 & -0.02  & \multirow{2}{*}{3} & \textbf{0.09} & 0.01 & 0.02 \\
&&  & -0.08  &  -0.0 & 0.0  &   &  -0.03 & -0.02 & -0.02   &  &  -0.01 & -0.03 & -0.02  &  &  -0.04 & -0.03 & -0.02  \\\cline{2-18}


&\multirow{2}{*}{Law School}& \multirow{2}{*}{3} &   0.01 & -0.0 & 0.0  & \multirow{2}{*}{4} &0.0 & 0.0 & 0.0  & \multirow{2}{*}{2} &  0.0 & -0.0 & 0.0  & \multirow{2}{*}{1} &  0.01 & 0.0 & 0.0 \\
&&&  -0.0 & 0.0 & 0.0 & & -0.0 & 0.0 & 0.0 & & -0.02 & 0.0 & 0.0 & & -0.0 & 0.0 & 0.0  \\\cline{2-18}


&\multirow{2}{*}{Student}& \multirow{2}{*}{0} &  0.0 & 0.0 & 0.0  & \multirow{2}{*}{0} & 0.0 & 0.0 & 0.0  & \multirow{2}{*}{1} &  0.01 & -0.01 & -0.01  & \multirow{2}{*}{0} &0.0 & 0.0 & 0.0 \\
&&&  -0.0 & 0.0 & 0.0 & & -0.0 & 0.0 & 0.0 & & -0.01 & -0.02 & -0.01 & & -0.0 & 0.0 & 0.0 \\\cline{2-18}


&\multirow{2}{*}{Heart}& \multirow{2}{*}{1} & 0.01 & 0.0 & 0.0  & \multirow{2}{*}{1} & 0.01 & 0.0 & 0.0  & \multirow{2}{*}{1} & \textbf{0.02} & 0.0 & 0.01 & \multirow{2}{*}{1} & 0.0 & 0.0 & 0.01 \\
&&&  -0.02 & 0.0 & -0.0 & & -0.01 & 0.0 & -0.0 & & -0.1 & 0.02 & -0.02 & & -0.0 & 0.0 & 0.0 \\\cline{2-18}

\hline
\end{tabular}
\vspace{-1.0 em}
}
\label{tab:distribution_shift}
\end{table*}


==> Sections/table_drop_non_sens.tex <==

% {\footnotesize
\begin{table}[t]
\caption{Non-Sensitive Feature Selection Methods and Their Local Robustness.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabu}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multirow{2}{2.5em}{\textbf{Dataset}}  &\multicolumn{4}{| c |}{\hfil\textsc{SelectKBest}} & \multicolumn{4}{| c |}{\hfil\textsc{SelectFpr}}  &\multicolumn{4}{| c |} {\hfil\textsc{SelectPercentile}} \\\cline{2-13}
&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}&\hfil\texttt{\#Edge diff}&\hfil\texttt{EOD diff}&\hfil\texttt{Acc diff} &\hfil\texttt{F1 diff}   \\
\hline

\multirow{2}{*}{Adult}& 4 & \textbf{0.05} & -0.01 & -0.01 &  4 & \textbf{0.02} & 0.0 & 0.0 & 4 & \textbf{0.35} & -0.09 & -0.14 \\
& 4 & -0.13 & -0.01 & -0.04 &  4 & -0.13 & -0.01 & -0.04 & 4 & -0.06 & -0.04 & -0.12 \\
\hline

\multirow{2}{*}{Compas} & 3 & \textbf{0.1} & -0.0 & -0.0 &  3 & \textbf{0.1} & 0.0 & -0.0 & 3 & \textbf{0.12} & -0.02 & -0.02 \\
& 2 & -0.02 & 0.0 & -0.0 &  2 & -0.04 & 0.0 & -0.0 & 2 & -0.07 & -0.01 & 0.0 \\
\hline

\multirow{2}{*}{Bank}& 1 & \textbf{0.1} & -0.08 & -0.05 &  2 & \textbf{0.06} & -0.01 & 0.0 & 1 & \textbf{0.15} & -0.08 & -0.6 \\
& 2 & -0.05 & -0.07 & -0.23 &  2 & -0.0 & 0.0 & 0.0 & 2 & -0.36 & -0.03 & -0.13 \\
\hline

\multirow{2}{*}{Law School}&  1 & \textbf{0.04} & -0.0 & -0.0 &  0 & \textbf{0.0} & 0.0 & 0.0 & 0 & \textbf{0.02} & -0.0 & -0.0 \\
& 1 & 0.0 & -0.0 & -0.0 &  0 & 0.0 & 0.0 & 0.0 & 1 & -0.01 & -0.01 & -0.01 \\
\hline

\multirow{2}{*}{Student}&  0 & \textbf{0.01} & -0.0 & 0.0 &  8 & \textbf{0.01} & -0.01 & -0.01 & 0 & \textbf{0.02} & -0.02 & -0.01 \\
& 8 & -0.01 & -0.01 & -0.0 &  8 & -0.02 & -0.0 & -0.0 & 8 & -0.01 & -0.02 & -0.02 \\
\hline

\multirow{2}{*}{Heart}&  1 & \textbf{0.04} & -0.02 & -0.03 &  1 & \textbf{0.02} & -0.0 & -0.01 & 2 & \textbf{0.16} & -0.07 & -0.23 \\
& 1 & -0.02 & -0.01 & -0.02 &  0 & -0.02 & -0.02 & -0.08 & 1 & -0.01 & -0.03 & -0.1 \\
\hline
\end{tabu}
}
\label{tab:table_drop_nonsens}
\end{table}
% }




%\begin{table*}[ht]
%\centering
%\resizebox{\textwidth}{!}{
%\begin{tabu}{|cc|}
%\hline

%Dataset & Perturbed edge& \texttt{$step\_size$}& \multirow{2}{*}$SelectKBest$&\multirow{2}{*}$SelectFpr$& \multirow{2}{*}$SelectPercentile$\\

%& & & $(EOD,Acc,F1)$ &$(EOD,Acc,F1)$&$(EOD,Acc,F1)$\\
%\hline

%$Insurance$& $education -> income$ & -1.21$&+0.083,-0.01,-0.01$&&\\
%$Insurance$ & $race -> education$ & +3.73$ &-0.069,-0.02,-0.01$  &&\\
%\hline
%Adult& race -> high income &$0.03$&  &&\\
%Adult& education -> hours-per-week & $0.04$ &&&\\

%\hline
%Compas & sex -> juvenile offense & +3.44$ &&&\\

%Compas & race -> reoffend & +0.01$ &&&\\

%\hline
%Law School & race - > pass exam & +3.29$&  &&\\
%Law School& race - > pass exam & +1.73$&  &&\\

%\hline

%\hline

%\end{tabu}
%}
%\caption{Results of dropping non-sensitive features}
%\label{tab:table_drop_nonsens}
%\end{table*}
%}
\begin{comment}
\multirow{2}{*}{Adult}& hours-per-week $\to$ workclass & -1.1 & \textbf{+0.12} & +0.05 & +0.05 & hours-per-week $\to$ workclass & -1.1 & \textbf{+0.10} & +0.05 &  +0.05  & hours-per-week $\to$ workclass & -1.1 & \textbf{+0.11} & +0.01 & +0.03 \\
& gender $\to$ education & +3.5 & -0.12 & +0.01 & +0.01 & gender $\to$ education & +3.5 & -0.13 & -0.01 & -0.01  & hours-per-week $\to$ workclass & +0.7 & -0.12 & -0.02 & -0.2 \\
\hline

\multirow{2}{*}{Compas} & race $\to$ juvenile\_offense & -1 & \textbf{+0.08} & -0.02 & -0.02 & age $\to$ degree\_charge & -0.3 & \textbf{+0.13} & -0.05 & -0.03 & race $\to$ reoffend & -0.92 & \textbf{+0.12} & -0.01 & -0.01 \\
& race $\to$ reoffend & +4.2  & -0.33 & -0.05 & -0.02 & race $\to$ reoffend & +4.2 & -0.21 & -0.04 & -0.02 & race $\to$ reoffend & +4.2 & -0.44 & -0.03 &-0.02 \\
\hline
\multirow{2}{*}{Law School}& race $\to$ pass~exam & +5.0 & \textbf{+0.07} & -0.01 & -0.05 & race $\to$ pass~exam & +5.0  & \textbf{+0.02} & 0.0 & -0.02 &  race $\to$ pass~exam & +5.0  & \textbf{+0.04} & 0.0 & -0.05 \\
& race $\to$ pass~exam & -4.4 & -0.23 & -0.01 & -0.01 &  race $\to$ pass~exam & -4.4 & -0.22& -0.01 & -0.01 &  race $\to$ pass~exam & -4.9 & -0.12 & -0.01 & -0.01 \\
\hline

\multirow{2}{*}{Student}& sex $\to$ G1 & -5.0 & \textbf{+0.19} & -0.01 & -0.01 & sex $\to$ G1 & -5.0 & \textbf{+0.15} & -0.01 & -0.02 & sex $\to$ G1 & -5.0 & \textbf{+0.34} & -0.04 & -0.07 \\
& sex $\to$ failures & +0.2 & -0.12 & -0.02 & -0.01 & sex $\to$ failures & +0.2 & -0.11 & -0.02 & -0.01 & sex $\to$ failures & +0.2 & -0.13 & -0.02 & -0.01 \\
\hline
\end{comment}

==> Sections/table_drop_sens.tex <==
\begin{table}[t]
\caption{Results of dropping sensitive features.}
\label{tab:table_drop_sens}
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{|cccccc|}
\hline
Dataset & \#Edge diff &  sensitive feat & EOD diff & Acc diff & F1 diff \\ 
\hline

\multirow{2}{*}{Adult} & 3 & sex & \textbf{0.09} & 0.09 & -0.03 \\
 & 4 & sex & -0.13 & -0.01 & -0.04 \\
\hline
\multirow{2}{*}{Compas}& 3 & race & \textbf{0.11} & 0.09 & 0.0 \\
 & 2 & race & -0.04 & 0.0 & 0.0 \\

\hline

\multirow{2}{*}{Bank} & 1 & age & \textbf{0.11} & 0.09 & -0.24 \\
 & 0 & age & -0.06 & -0.03 & -0.02 \\
\hline
\multirow{2}{*}{Law School }&0 & sex & \textbf{0.04} & -0.02 & 0.0 \\
 & 1 & sex & 0.01 & 0.0 & 0.0 \\
\hline

\multirow{2}{*}{Student} & 8 & sex & \textbf{0.01} & 0.01 & 0.0 \\
 & 8 & sex & -0.01 & -0.0 & 0.0 \\
\hline

\multirow{2}{*}{Heart} & 1 & sex & \textbf{0.05} & -0.04 & -0.0 \\
 & 2 & sex & -0.02 & 0.0 & 0.0 \\
\hline
\end{tabular}
}
\end{table}

